Visual Deprojection: Probabilistic Recovery of Collapsed Dimensions

We introduce visual deprojection: the task of recovering an image or video that has been collapsed along a dimension. Projections arise in various contexts, such as long-exposure photography, where a dynamic scene is collapsed in time to produce a motion-blurred image, and corner cameras, where reflected light from a scene is collapsed along a spatial dimension because of an edge occluder to yield a 1D video. Deprojection is ill-posed-- often there are many plausible solutions for a given input. We first propose a probabilistic model capturing the ambiguity of the task. We then present a variational inference strategy using convolutional neural networks as functional approximators. Sampling from the inference network at test time yields plausible candidates from the distribution of original signals that are consistent with a given input projection. We evaluate the method on several datasets for both spatial and temporal deprojection tasks. We first demonstrate the method can recover human gait videos and face images from spatial projections, and then show that it can recover videos of moving digits from dramatically motion-blurred images obtained via temporal projection.

==> motivation.tex <==
\section{Notation and Preliminaries}
\label{sec:motivation}
Let ${(\bx^i, \by^i)}_{i=1}^N$ be a collection of pairs of projections $\bx \in R^d$, and true signals $\by \in R^D$. We assume an unknown projection function $f_{\omega}(\cdot)$, that collapses $\by$ along a dimension to produce $\bx$: 

\begin{equation}
\bx^i = f_{\omega}(\by^i) + \epsilon^i,  
\end{equation}

where $\omega$ are function parameters and $\epsilon^i ~\sim N(0, \mathbf{I}\sigma_x^2)$ is a noise term. We focus on the most practical case where $f_{\omega}(\cdot)$ is a linear operation, such as averaging a signal along a dimension.
%$\bx = \sum_{t=1}^T \omega_t  \by_t + \epsilon$, where $w_t = \frac{1}{T},$ $\forall t$.



\begin{figure}[h!]
\begin{center}
\includegraphics[width=\linewidth]{figures/discrete_examples.pdf}
\end{center}
\caption{Examples of the types of variability for the deprojection task in our datasets.}
\label{fig:discrete_examples}
\end{figure}

There are many plausible $\by$ candidates from which an $\bx$ may have been generated. We would therefore like to capture the distribution $p(\by | \bx)$, and not just a single estimate. To motivate our work, we first discuss a simpler approach to tackle this problem. Consider the simple case where $E[Y | X = \bx]$ is a linear function of $\bx$: $E[Y | X = \bx] = A\bx + b$ with matrices $A$ and vector $b$. It is straightforward to derive the MMSE (minimum mean squared error) estimator for $p(\by | \bx)$:
\begin{equation}
\footnotesize
p(\by | \bx)= \mathcal{N}(\by; \Sigma_{YX}\Sigma_X^{-1}(\bx - \hat{\bx}) + \hat{\by}, \Sigma_{Y} - \Sigma_{YX}\Sigma_X^{-1}\Sigma^T_{YX}), 
\label{eq:mmse}
 \end{equation}
where $\Sigma_X$ and $\Sigma_Y$ are the covariance matrices of $X$ and $Y$ and $\Sigma_{XY}$ is their cross-covariance matrix [cite]. The only requirement to use this estimator is that X and Y have well-defined first and second moments, though the ideal case is when X and Y are Gaussian. 

\begin{figure}[h!]
\begin{center}
\includegraphics[width=2.5in]{figures/mnist_mmse.pdf}
\end{center}
\caption{Sample results using the linear MMSE estimator. Each row is a different example, and the input horizontal projections (averages) of MNIST digits and the true images are shown in leftmost columns. Three sampled images from the MMSE estimator per example are shown in the remaining columns.}
\label{fig:discrete_examples}
\end{figure}

Fig. shows examples of sampling from the MMSE model to deproject horizontal projections of the MNIST~\cite{mnist} dataset of handwritten digits. Notice how the estimated tends to produce blurry outputs. This is because the assumption of joint Gaussianity of the vectorized inputs is not appropriate. For a given input projection, digits of varying classes and characteristics may be produced. This effect is more pronounced on more complex datasets. We present a method that learns a more appropriate embedding for a given dataset using neural network function approximators. Sampling from this model will allows us to produce more realistic outputs. 
